Hardware Acceleration of Neural Graphics

Rendering and inverse-rendering algorithms that drive conventional computer graphics have recently been superseded by neural representations (NR). NRs have recently been used to learn the geometric and the material properties of the scenes and use the information to synthesize photorealistic imagery, thereby promising a replacement for traditional rendering algorithms with scalable quality and predictable performance. In this work we ask the question: Does neural graphics (NG) need hardware support? We studied representative NG applications showing that, if we want to render 4k res. at 60FPS there is a gap of 1.5X-55X in the desired performance on current GPUs. For AR/VR applications, there is an even larger gap of 2-4 OOM between the desired performance and the required system power. We identify that the input encoding and the MLP kernels are the performance bottlenecks, consuming 72%,60% and 59% of application time for multi res. hashgrid, multi res. densegrid and low res. densegrid encodings, respectively. We propose a NG processing cluster, a scalable and flexible hardware architecture that directly accelerates the input encoding and MLP kernels through dedicated engines and supports a wide range of NG applications. We also accelerate the rest of the kernels by fusing them together in Vulkan, which leads to 9.94X kernel-level performance improvement compared to un-fused implementation of the pre-processing and the post-processing kernels. Our results show that, NGPC gives up to 58X end-to-end application-level performance improvement, for multi res. hashgrid encoding on average across the four NG applications, the performance benefits are 12X,20X,33X and 39X for the scaling factor of 8,16,32 and 64, respectively. Our results show that with multi res. hashgrid encoding, NGPC enables the rendering of 4k res. at 30FPS for NeRF and 8k res. at 120FPS for all our other NG applications.

==> arch_old.tex <==
\label{sec:arch}
We performed the breakdown analysis of the 
representative 
\nG applications for different 
\IE types, 
to identify 
the kernels that 
consume most of the 
cycles(Section~\ref{sec:understandingPerf}). 
Figure~\ref{fig:app_brkdn} presents the 
cycle consumption breakdown for different 
kernels of neural graphics applications for 
different input encoding types. 
Our analysis shows that, 
for \ieOne \IE, on average 
across all four \nG applications 
\iePercentHashgrid 
cycles are consumed by the \IE kernel
and \mlpPercentHashgrid cycles are consumed
by the \MLP kernel. 
For \ieTwo \IE, on average 
across all four \nG applications 
\iePercentDensegrid
cycles are consumed by the \IE kernel
and \mlpPercentDensegrid cycles are consumed
by the \MLP kernel. 
Similarly, for \ieThree \IE, on average 
across all four \nG applications \iePercentDensegridLowRes 
cycles are consumed by the \IE kernel
and \mlpPercentDensegridLowRes cycles are consumed
by the \MLP kernel. 
Hence, the \IE 
and the \MLP are the two most expensive 
kernels across all four representative neural 
graphics applications. 
This is expected behaviour, as 
the algorithmic 
analysis of the \nG applications, 
explained in the 
section~\ref{sec:understandingPerf},
suggests
that the input encoding and the \MLP 
are the two major building blocks of the 
\nG applications. 
This motivates the need to accelerate 
the \IE and \MLP kernels. Hence, we designed 
the architecture to accelerate  
the \IE and \MLP kernels in hardware. \\

We also performed the detailed breakdown analysis
of the \IE kernel for different 
\IE types, in order to understand the 
bottlenecks 
(Section~\ref{sec:understandingPerf}). 
Figure~\ref{fig:IE_brkdn} shows the cycle 
level breakdown of the five 
most expensive operations. 
As explained in the 
section~\ref{sec:understandingPerf}
the grid lookups are the 
major building blocks of the \IE algorithms,
our analysis also shows that 
the grid lookups take significant amount 
of cycles across all three \IE types. 
This is because the GPU are usually more 
efficient for compute intensive tasks than 
memory intensive tasks 
and grid lookup is a 
memory intensive task which does not utilize the 
compute capabilities of the GPU as can be seen 
in Table~\ref{tab:} the compute utilization 
of GPU is very low for \IE kernel. 
Moreover, the lookup tables for all the 
resolutions
do not entirely fit 
on the L2 cache of RTX3090 
and the memory wait time to resolve 
the caches misses 
is also adding
to the overall cycles. 
Our analysis also shows that, 
in all three \IE types 
the 
integer mapped modulo operation
are one of the most expensive operations. 
This is because the 
modulo operation gets mapped to the
general purpose
ALU of the GPU and can not 
utilize the efficient tensor cores of the GPU.

As \ieTwo and \ieThree have one-on-one 
mapping of grid indices, the hash function 
is not called for these \IE types and hence the 
breakdown shows zero cycles for hash 
function. However, hash function 
consumes significant amount of cycles 
for \ieOne. 
This is because the hash function
requires \xor operation which can not 
exploit the efficient tensor cores of the GPU 
and is rather scheduled on the 
general purpose ALU of the GPU.

As shown in the \IE breakdown 
(Figure~\ref{fig:IE_brkdn})
other relatively simpler compute operations 
also consume significant amount of cycles
because they have to wait for the grid-lookup 
memory 
requests to get resolved.
%for the grid lookups.
The kernel level breakdown analysis 
motivates the need to provide hardware 
support to accelerate modulo operation, 
grid lookups and the dataflow of the 
\IE to accelerate \IE kernel in hardware. 
Moreover, in neural graphics 
applications the outputs of the \IE kernel
are always consumed by the \MLP kernel. 
Whereas, our analysis of the GPU based 
scheduling of the neural graphics application 
shows that in Nvidia's implementation
of these applications~\ref{instant-ngp} 
the outputs of the 
\IE kernel are written to the device memory 
and then fetched back by the \MLP kernel.
This is because the \IE and \MLP are 
implemented as separate 
CUDA kernels and the CUDA kernel corresponding 
to the \IE deposits data to the global memory 
and the CUDA kernel corresponding to the 
\MLP picks up that data from global memory.
Figure~\ref{fig:app_gpu} shows 
mapping of a typical neural graphics application
on a GPU. As highlighted in the figure, the \IE 
kernel writes outputs to device memory and 
the \MLP kernel fetches that data again for 
further processing. 
This leads to unnecessary memory traffic and 
waste of energy for DRAM accesses that can 
potentially be avoided. 
This opportunity can be exploited in the 
hardware by fusing the \IE and \MLP 
engines in such a way that the \IE engine 
directly writes the outputs to the input memory 
of the \MLP engine. \\

In order to accelerate the two most 
expensive
primitives of the \nG applications (\IE and 
\MLP), we present a \NFP in 
Figure~\ref{fig:arch}.
The \NFP architecture 
%, presented in 
%Figure~\ref{fig:arch}
is inspired by the insights learned from the
breakdown analysis of the \nG applications. 
Each \NFP has an \IE IP and an \MLP 
engine fused together in hardware. 
The Figure~\ref{fig:arch}-a presents 
the architecture of the \IE IP. 
Each \IE IP has a dedicated 
on-chip SRAM (\emph{grid\_sram}) to cache the 
lookup 
table for 
one resolution level.
The size of the \emph{grid\_sram} 
(1MB per \IE IP)
is chosen such that 
the entire lookup table for one resolution
level fits on the on-chip SRAM, and the 
off-chip memory access penalty
could be avoided for grid lookups. 
The lookup table for one resolution level is 
cached once on the dedicated 
\emph{grid\_sram} of one \IE IP and then lookups 
are performed for all the inputs 
for the entire frame. 
Our hardware architecture has 16
\IE IPs to matched the maximum number of 
resolution 
levels of the \nG applications. 
As the \ieOne \IE has 16 resolution levels,
each of the 16 \IE IPs caches the lookup table 
corresponding to one resolution level and then
performs the \IE for all the resolution 
levels in parallel.
As \ieTwo \IE has 8 resolution levels, 
two inputs can be processed in parallel. 
Similarly, as \ieThree \IE has 2 resolution 
levels, the \IE IP can process 8 inputs 
in parallel. 
The architecture of the \IE IP is shown
in Figure~\ref{fig:arch}-a, 
the normalized input coordinates 
are pre-fetched into 
the input FIFO.
The \emph{grid\_scale} module calculates the 
scale of the grid from the base-resolution of 
the grid and the resoltion 
level being processed. 
The \emph{pos\_fract} module is responsible 
for converting the normalized input 
coordinates to the absolute 
coordinates. It multiplies the 
normalized coordinates with grid scale 
to compute the absolute coordinates, which are
then
passed to the
\emph{grid\_index} module for the index 
calculation. 
The \emph{grid\_index} module is responsible for 
calculating the final indices for 
the lookup operations.
As shown in Figure~\ref{fig:arch}-a, the 
\emph{grid\_index} module can be 
configured to either hash in the indices
for the \ieOne encoding or compute the indices 
without the hashing function for the \ieTwo
and \ieThree encoding types. 
The algorithm to compute the indices for the 
lookup operation,
takes the 
modulo of the indices with the 
hash-map size,
as an intermediate operation, 
before the final indices could be calculated.
We observed that the hash-map size 
is always power of two for all our \nG
applications, 
we exploit this optimization opportunity in 
hardware and approximate the modulo operation 
with shift operation in \IE IP. 
The final outputs of the \emph{grid\_index} 
modules are actual indices that are directly 
used to perform the feature lookups from the 
\emph{grid\_sram}. The \emph{interpol\_weights}
module 
computes the interpolation weights that are then
multiplied with the features to compute the 
final features that fed to the \MLP engine. 
The data-flow and the corresponding compute 
operations of each module of the \IE IP
are shown in Figure~\ref{fig:arch}-a.
As each \IE IP calculates features for one 
resolution level, the outputs of the 
\IE IPs are concatenated together to get the 
final input vector for the MLP engine. 
The structure of the \MLP for 
all the \nG applications is shown in 
Table~\ref{tab:app_struct}. 
We observed that
the \MLP in all the \nG applications have 
2-4 hidden layers and the number of hidden 
neurons is always 64 in each hidden layer of the 
\MLP.
This is because part of the learning 
task is offloaded to the learn-able 
parameters of \IE and relatively 
smaller \MLP with only 2-4 hidden layers and 
small number of hidden neurons (64 hidden 
neurons per layer) are enough to synthesize good 
quality output images. 
Based on this observation we have a 
$64\times64$ grid of MAC units that computes 
one layer of the \MLP at a time.
As the size of the hidden layer is relatively 
small, a dedicated small on-chip SRAM is
used to store the 
intermediate features of the hidden layers. 
Keeping the intermediate features on-chip, 
removes the off-chip memory accesses 
for storing/fetching the intermediate features 
and improves the performance by 1OOM 
~\cite{nrc}. \\
Figure~\ref{fig:gpu_interact}-a shows the 
interaction of the \NFP with the GPU. 
A conventional Nvidia GPU has Graphics 
processing clusters (GPC) that have multiple 
streaming processors (SMs) connected to a 
shared L2 cache. 
We propose a scalable \NPC (\npc) along with 
the existing GPC units. The proposed \npc is 
connected to the shared L2 cache, and can 
be scaled to have N number of \nfp units. 
Figure~\ref{fig:gpu_interact}-b 
and~\ref{fig:gpu_interact}-c show the 
programming model of the \npc. 
The command processor 
(Giga Thread Engine in Nvidia's terminology)
schedules the CUDA kernel on the streaming multiprocessors by 
clustering the streaming multiprocessors
in blocks.
We propose a similar programming model 
for the \npc, where the command buffer 
configures the \npc and schedules the 
\IE and the \MLP kernels on the \npc.
The rest of the kernels are scheduled 
just as conventional CUDA program 
on the streaming multiprocessors.
The outputs of the \npc are written back 
to the GPU memory, and are read by the 
streaming multiprocessors, which then compute 
the rest of the kernels.  
The inputs are divided into batches,
while the GPU is processing the rest of the 
\nG application kernels for the Nth batch of 
inputs, the N+1st batch is scheduled on the 
\npc to compute the \IE and MLP
kernels in parallel, as shown in 
Figure~\ref{fig:gpu_interact}-b. 

%\begin{itemize}
%    \item arch F-a arch [table:IE ip steady state]
%    \item interaction F-b interaction
%    \item programming 
%    \item F-c programming multiple IPs multiple copies
    
%\end{itemize}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{architecture.drawio.png}
    \caption{Neural Fields Processor (NF-P)}
    \label{fig:arch}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{gpu_interaction.drawio.png}
    \caption{Interaction with the GPU.}
    \label{fig:gpu_interact}
\end{figure*}




==> myvalidation.tex <==
\textcolor{red}{
ahmdl's law 
use timeloop/accelergy to 
}

==> neuralGraphics.tex <==
\label{sec:neuralGraphics}


Figure~\ref{fig:cgvsng} shows a high level 
comparison between the conventional computer 
graphics based rendering pipeline and 
the neural graphics based rendering pipeline.
Rendering in conventional computer graphics starts with 
the detailed description of the physical and material properties 
of the scene and the camera.
This description is passed as input to the rendering 
pipeline which then generates a 2D image/frame as output.
\iffalse
Rendering pipeline in conventional computer graphics 
consists of a series of programmable and fixed function 
stages. 
%Stages with a green color are known as 
The fixed-function stages (shown as blue in the 
Figure~\ref{fig:cgvsng}) are the predefined stages which 
can be slightly tweaked by using input parameters, 
however their functionality is fixed. 
%However, 
The operations of the programmable stages 
(shown as yellow in the Figure~\ref{fig:cgvsng}) can be 
completely defined by the programmer. 
E.g. custom code can implemented for the shader stages
to implement anything from 
texturing and lighting to ray tracing.
Rendering pipeline in conventional computer graphics 
starts with the 
\emph{input assembler} which is a fixed-function stage 
and collects the raw vertex data from the 
specified buffers. 
Then \emph{vertex shader} runs for every vertex 
and turns vertex positions from 
model space to screen space. 
The \emph{vertex shader} stage is programmable and 
is also responsible for passing the 
per-vertex data down the rendering pipeline.
The goal of the \emph{tessellation} and the 
\emph{geometry shader} stages is 
to increase the mesh quality.
These are programmable stages and 
run on every primitive (triangle, line, point). 
Certain rules can be specified in these stages to 
subdivide the geometry 
and to discard primitives or output more primitives than came in. 
The \emph{rasterization} is a fixed-function stage 
and is responsible for discretizing the primitives 
into fragments. 
These fragments 
are the pixel elements that will fill the framebuffer.
The \emph{rasterization} stage is also responsible for 
discarding the fragments 
that are outside the screen area or behind other 
primitive fragments, which is achieved by 
depth testing.
After \emph{rasterization}, the 
the \emph{fragment shader} is invoked for every fragment 
and is responsible for identifying the corresponding 
framebuffer(s) that the fragments should map to,
and determining the final color and depth values
for the fragments. 
Once the fragments are mapped to the corresponding framebuffer,
a fixed-function \emph{color blending} stage 
mixes the fragments that map to the same pixels 
in a framebuffer. 
This is the final stage of the 
rendering pipeline where once the colors of the fragments are 
mixed, usually based on their transparency values, 
the final frame is ready to be displayed.
\fi
%Figure~\ref{fig:cgvsng} also shows the 
%graphics pipeline based rendering alternative (neural rendering).
In neural rendering, a detailed description of the 
physical and material properties of the scene can be avoided, 
rather a few scene observations (images or video) are used as 
input to the neural rendering pipeline. 
Neural graphics also replaces the conventional 
rendering pipeline with much simpler 
neural rendering pipeline.
The neural rendering pipeline at high level consists 
of three stages 1) {\em Pre-processing stage} which is 
responsible for generating the actual input features for the 
neural networks from the given positional coordinates.
2) {\em The fully-connected neural network stage} that actually 
computes the forward pass of the fully-connected neural 
networks 
and outputs the 
color and density values corresponding to the input features.
3) {\em The output accumulation stage} that accumulates 
the color and density values to generate the final 
pixels to be displayed. 
Section~\ref{sec:understandingPerf} provides further 
details about these stages. \\

Figure~\ref{fig:cgvsngbenefits} shows the 
high level benefits of neural graphics over conventional
computer graphics. 
1) {\bf More compact representations of scenes:}
In classical computer graphics, "Fields" are widely 
used to 
parameterize the physical properties of an
object or scene over space and time.
Such space-time parameterizations, defined for all spatial 
and/or temporal coordinates, are  
needed to synthesize 3D
shapes and/or 2D images.
%By definition,
%A field is a quantity defined for all spatial 
%and/or temporal coordinates"~\cite{}.
%In computer graphics, we are usually 
%interested in scalar and vector fields such as 
The fields of interest include images (vector fields), occupancy fields (scalar fields), 3D/2D 
shapes/geometries (scalar fields), and signed distance 
fields (scalar fields).
Continuous functions are typically used to faithfully
represent a field in computer graphics. 
These continuous functions are then 
sampled and stored as discrete samples
in computers. 
The sampling rate must be at least the Nyquist sampling rate
to avoid aliasing. 
In classical computer graphics, as the complexity of the scene 
grows, the memory requirement to store these samples 
explodes. 
However, 
in neural graphics, the field is parameterized, 
fully or in part,
by a neural network. Such parameterized fields are known as 
neural fields.
The parameters of neural networks are inherently 
continuous and does not require Nyquist sampling for storage.
Hence, neural fields enable compact and efficient 
representations of the scene.
%compared to conventional computer graphics.
%neural networks can be used for 
%compact representations of continuous functions.
2) {\bf Simpler and domain agnostic data structures:} 
In conventional computer graphics, 
complex data structures such as 3D point clouds, 3D meshes,
voxel based 3D models, parametric models,
and depth maps are used  
for 3D representations. 
These data structures are scene geometry dependent.
Whereas, in neural graphics, the 3D scenes are learned 
in the weights of the neural networks.
These weights are stored as matrices which are 
much simpler data structures compared to 
conventional 3D representations.
%3D point clouds, 3D meshes,
%voxel based 3D models, parametric models,
%and depth maps. 
Moreover, unlike conventional 3D representations, 
the weight matrices of a neural network are scene geometry 
agnostic. 
3) {\bf Deterministic rendering time:}
In conventional computer graphics, the rendering time is 
non-deterministic as it 
depends upon the complexity of the scene.
In neural graphics, as "rendering" is effectively 
replaced by the inference operation of the neural networks, the
rendering time is deterministic as the inference time 
of neural networks is 
inherently
deterministic.
4) {\bf Simpler scene definition:}
As explained earlier, in conventional computer graphics 
a complete description of the physical and material properties of
the scene is required for rendering. In neural graphics, however, 
the properties of the scene can implicitly be learned from 
a few images or video of the scene. This leads to much simpler scene definitions.
%why? \\

The above benefits make neural graphics arguably the biggest advance in the field of computer graphics in decades.
 


%\begin{itemize}
%    \item what is it? 
%    \item why
%    \item types (applications)
%    \item F-a CG vs NG
%    \item F-b NG in systems benefits
%\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{CGvsNG.drawio.png}
    \caption{Rendering: Conventional Computer Graphics VS Neural Graphics}
    \label{fig:cgvsng}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{benefitsCGvsNG.drawio.png}
    \caption{Inherent benefits of Neural Graphics over 
    Conventional Computer Graphics}
    \label{fig:cgvsngbenefits}
\end{figure}

==> relatedWork.tex <==
\label{relatedWork}
Neural graphics is a rapidly emerging field with
1000s of papers written only in past couple of years.
Vanilla-NeRF~\cite{nerf} can be considered as the seminal work that 
sparked the recent interest in neural graphics.
Vanilla-NeRF trained a fully connected network by feeding it a series of images
of the scene taken from different camera positions and viewing angles. 
They showed that the model can learn the geometry and the light field of the 
scene and synthesize high fidelity images from novel camera view points. 
Vanilla NeRF~\cite{nerf} was also the first paper to 
use the concept of input encoding in the context of 
neural graphics. 
For neural networks, input encodings have proven useful in the 
recurrent networks~\cite{Gehring17} and transformers~\cite{Vaswani17}.
Vanilla-NeRF observed that the neural network fails to 
learn the high frequency variations in the color and 
the geometry of the scene when the network is trained by directly feeding the 
3D position coordinates and the 2D camera viewing angles.
In order to solve the learning problem, 
they mapped the 5D Vector of positions and viewing angle to higher 
dimensional space using high frequency sinusoidal functions.
The simplicity and impressive results
inspired many adaptations to the vanilla-NeRF, 
sometimes being referred to as the NeRF explosion~\cite{DY21}.
The followup papers of vanilla-NeRF showed that the 
neural networks along with input encoding 
can be used for a wide range of applications. 

The followup research presented NeRF varaints 
to capture dynamic free-viewpoint video~\cite{PSB*20, LNSW21, XHKK20, PCPM21, DZY*20}, 
generate photorealistic avatars~\cite{GTZN21, GSL*20, LSS*21}, 
perform relighting on captured scenes~\cite{MRS*21, BXS*20, SDZ*21, BBJ*20},
conditionally encode shape and appearance via latent codes~\cite{SLNG20, CMK*21, YYTK21, TY20}  
and
compose scenes of multiple objects ~\cite{OMT*21,YLSL21,NG21}. 
There had been several recent publications on improving the run-time of NeRF on modern GPUs.
Neural sparse voxel fields (NSVFs)~\cite{LGZ*20} 
used a self-pruning sparse voxel octree structure
that to enable the empty space skipping 
which reduces the number of neural network queries and improves the run-time of their NeRF variant. 
Alternatively, ~\cite{LMW21} learns the 
partial integrals,
to reduce the number of evaluations
along a ray. ~\cite{RJY*20} decompose the scene with a
Voronoi decomposition to train multiple NeRFs for each cell
and effectively improve the performance of NeRF.
Although these NeRF variants show impressive quality, the 
huge computational cost of these algorithms makes them unsuitable for
real-time applications.

Many works tried to improve the input encoding algorithms to 
improve the overall quality and performance of the NeRF vasriants. 

Instant-NGP~\cite{ngp} can be considered as the state of the art in the neural graphics at the moment. 
They proposed 
\ieOne encoding that enables tiny neural networks to capture complex scenes.
Using \ieOne encoding and tiny neural networks they 
achieved state of the art training and inference times while maintaining 
high visual fidelity. 
To the best of our knowledge, there does not exist any peer-reviewed domain specific 
architectures to accelerate neural graphics. 
All of the above mentioned NeRF variants run on modern desktop class GPUs.


%\begin{itemize}
%    \item algorithms 
%    \item applications / SW
%    \item system / HW
%\end{itemize}

==> tabprep.tex <==
\begin{table}[]
\tiny
\centering
\caption{}
\label{tab:app_struct}
\begin{tabular}{@{}|c|c|@{}}
\toprule
Application               & Parameters                                                                                                                                                                                                                                                                                                                                   \\ \midrule
NeRF multi res. hashgrid  & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.51572 F=2 T=2\textasciicircum{}19 L=16 \\ Density model: 3--{[}HashGrid{]}--\textgreater{}32--{[}FullyFusedMLP(neurons=64;layers=3){]}--\textgreater{}1 \\ Color model: 3--{[}Composite{]}--\textgreater{}16+16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}3\end{tabular} \\ \midrule
NeRF multi res. densegrid & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.405 F=2 T=2\textasciicircum{}19 L=8 \\ Density model: 3--{[}DenseGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=3){]}--\textgreater{}1 \\ Color model: 3--{[}Composite{]}--\textgreater{}16+16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}3\end{tabular}   \\ \midrule
NeRF low res. densegrid   & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=128 b=1 F=8 T=2\textasciicircum{}19 L=2 \\ Density model: 3--{[}TiledGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=3){]}--\textgreater{}1 \\ Color model: 3--{[}Composite{]}--\textgreater{}16+16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}3\end{tabular}      \\ \midrule
NSDF multi res. hashgrid   & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.38191 F=2 T=2\textasciicircum{}19 L=16 \\ Model: 3--{[}HashGrid{]}--\textgreater{}32--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}1\end{tabular}                                                                                                                            \\ \midrule
NSDF multi res. densegrid  & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.405 F=2 T=2\textasciicircum{}19 L=8 \\ Model: 3--{[}DenseGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}1\end{tabular}                                                                                                                              \\ \midrule
NSDF low res. densegrid    & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=128 b=1 F=8 T=2\textasciicircum{}19 L=2 \\ Model: 3--{[}TiledGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}1\end{tabular}                                                                                                                                 \\ \midrule
NVR multi res. hashgrid  & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.275 F=2 T=2\textasciicircum{}19 L=16 \\ Model: 3--{[}HashGrid{]}--\textgreater{}32--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}4\end{tabular}                                                                                                                              \\ \midrule
NVR multi res. densegrid & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.405 F=2 T=2\textasciicircum{}19 L=8 \\ Model: 3--{[}DenseGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}4\end{tabular}                                                                                                                              \\ \midrule
NVR low res. densegrid   & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=128 b=1 F=8 T=2\textasciicircum{}19 L=2 \\ Model: 3--{[}TiledGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}4\end{tabular}                                                                                                                                 \\ \midrule
GIA multi res. hashgrid  & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.25992 F=2 T=2\textasciicircum{}24 L=16 \\ Model: 2--{[}HashGrid{]}--\textgreater{}32--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}3\end{tabular}                                                                                                                            \\ \midrule
GIA multi res. densegrid & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=16 b=1.405 F=2 T=2\textasciicircum{}24 L=8 \\ Model: 2--{[}DenseGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}3\end{tabular}                                                                                                                              \\ \midrule
GIA low res. densegrid   & \begin{tabular}[c]{@{}c@{}}GridEncoding: Nmin=128 b=1 F=8 T=2\textasciicircum{}24 L=2\\  Model: 2--{[}TiledGrid{]}--\textgreater{}16--{[}FullyFusedMLP(neurons=64;layers=4){]}--\textgreater{}3\end{tabular}                                                                                                                                 \\ \bottomrule
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\tiny
\centering
\caption{}
\label{tab:util}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                              &                                        &                                                                                             &                                                                                            &                                                                           &                                                                                                    &                                                                                                  \\
                              &                                        &                                                                                             &                                                                                            &                                                                           &                                                                                                    &                                                                                                  \\
\multirow{-3}{*}{App.-Kernel} & \multirow{-3}{*}{Grid Size/Block Size} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Comp. Util. \\ per kernel \\ call\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Mem. Util. \\ per kernel \\ call\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Kernel \\ Calls\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Comp. Util.\\ avg. across \\ application\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Mem. Util.\\ avg. across\\ application\end{tabular}} \\ \midrule
NeRF multi res. hashgrid      & (3853;16;1)/(512;1;1)                  & \cellcolor[HTML]{E06666}61.73                                                               & \cellcolor[HTML]{E06666}72.85                                                              & 59                                                                        & \cellcolor[HTML]{6AA84F}40.63                                                                      & \cellcolor[HTML]{E06666}72.02                                                                    \\
NeRF MLP                      & (3853;16;1)/(512;1;1)                  & \cellcolor[HTML]{6AA84F}34.3                                                                & \cellcolor[HTML]{E06666}65.2                                                               & 118                                                                       & \cellcolor[HTML]{6AA84F}33.36                                                                      & \cellcolor[HTML]{E06666}63.07                                                                    \\
NSDF multi res. hashgrid       & (1823;16;1)/(512;1;1)                  & \cellcolor[HTML]{E06666}73.08                                                               & \cellcolor[HTML]{6AA84F}43.54                                                              & 256                                                                       & \cellcolor[HTML]{93C47D}15.97                                                                      & \cellcolor[HTML]{6AA84F}30.8                                                                     \\
NSDF MLP                       & (1823;16;1)/(512;1;1)                  & \cellcolor[HTML]{6AA84F}38.13                                                               & \cellcolor[HTML]{E06666}71.74                                                              & 256                                                                       & \cellcolor[HTML]{93C47D}9.76                                                                       & \cellcolor[HTML]{93C47D}18.28                                                                    \\
NVR multi res. hashgrid       & (403;16;1)/(512;1;1)                   & \cellcolor[HTML]{E06666}52.5                                                                & \cellcolor[HTML]{E06666}59.03                                                              & 48                                                                        & \cellcolor[HTML]{93C47D}18.67                                                                      & \cellcolor[HTML]{6AA84F}30.36                                                                    \\
NVR MLP                       & (403;16;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}36.51                                                               & \cellcolor[HTML]{E06666}67.01                                                              & 48                                                                        & \cellcolor[HTML]{93C47D}11.51                                                                      & \cellcolor[HTML]{93C47D}21.05                                                                    \\
GIA multi res. hashgrid       & (4050;16;1)/(512;1;1)                  & \cellcolor[HTML]{CC0000}82.87                                                               & \cellcolor[HTML]{E06666}62.23                                                              & 1                                                                         & \cellcolor[HTML]{CC0000}82.87                                                                      & \cellcolor[HTML]{E06666}62.23                                                                    \\
GIA MLP                       & (4050;16;1)/(512;1;1)                  & \cellcolor[HTML]{6AA84F}39.1                                                                & \cellcolor[HTML]{E06666}72.22                                                              & 1                                                                         & \cellcolor[HTML]{6AA84F}39.1                                                                       & \cellcolor[HTML]{E06666}72.22                                                                    \\
NeRF multi res. densegrid     & (3966;8;1)/(512;1;1)                   & \cellcolor[HTML]{E06666}71.39                                                               & \cellcolor[HTML]{CC0000}91.81                                                              & 45                                                                        & \cellcolor[HTML]{E06666}57.37                                                                      & \cellcolor[HTML]{E06666}72.31                                                                    \\
NeRF MLP                      & (3966;8;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}39.53                                                               & \cellcolor[HTML]{E06666}68.4                                                               & 90                                                                        & \cellcolor[HTML]{6AA84F}34.51                                                                      & \cellcolor[HTML]{E06666}62.31                                                                    \\
NSDF multi res. densegrid      & (1823;8;1)/(512;1;1)                   & \cellcolor[HTML]{CC0000}76.1                                                                & \cellcolor[HTML]{6AA84F}48.25                                                              & 244                                                                       & \cellcolor[HTML]{93C47D}18.38                                                                      & \cellcolor[HTML]{93C47D}21.28                                                                    \\
NSDF MLP                       & (1823;8;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}41.66                                                               & \cellcolor[HTML]{E06666}73.49                                                              & 244                                                                       & \cellcolor[HTML]{93C47D}11.06                                                                      & \cellcolor[HTML]{93C47D}19.41                                                                    \\
NVR multi res. densegrid      & (403;8;1)/(512;1;1)                    & \cellcolor[HTML]{E06666}57.38                                                               & \cellcolor[HTML]{E06666}56.8                                                               & 48                                                                        & \cellcolor[HTML]{93C47D}17.41                                                                      & \cellcolor[HTML]{93C47D}22.43                                                                    \\
NVR MLP                       & (403;8;1)/(512;1;1)                    & \cellcolor[HTML]{6AA84F}39.83                                                               & \cellcolor[HTML]{E06666}67.67                                                              & 48                                                                        & \cellcolor[HTML]{93C47D}12.17                                                                      & \cellcolor[HTML]{93C47D}20.59                                                                    \\
GIA multi res. densegrid      & (4050;8;1)/(512;1;1)                   & \cellcolor[HTML]{CC0000}78.53                                                               & \cellcolor[HTML]{E06666}65.83                                                              & 1                                                                         & \cellcolor[HTML]{CC0000}78.53                                                                      & \cellcolor[HTML]{E06666}65.83                                                                    \\
GIA MLP                       & (4050;8;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}42.89                                                               & \cellcolor[HTML]{E06666}73.07                                                              & 1                                                                         & \cellcolor[HTML]{6AA84F}42.89                                                                      & \cellcolor[HTML]{E06666}73.07                                                                    \\
NeRF low res. densegrid       & (3980;2;1)/(512;1;1)                   & \cellcolor[HTML]{E06666}53.83                                                               & \cellcolor[HTML]{6AA84F}49.74                                                              & 43                                                                        & \cellcolor[HTML]{6AA84F}31.17                                                                      & \cellcolor[HTML]{E06666}59.57                                                                    \\
NeRF MLP                      & (3980;2;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}39.41                                                               & \cellcolor[HTML]{E06666}68.17                                                              & 86                                                                        & \cellcolor[HTML]{6AA84F}35.5                                                                       & \cellcolor[HTML]{E06666}64.1                                                                     \\
NSDF low res. densegrid        & (1823;2;1)/(512;1;1)                   & \cellcolor[HTML]{E06666}55.88                                                               & \cellcolor[HTML]{6AA84F}45.52                                                              & 260                                                                       & \cellcolor[HTML]{93C47D}7.21                                                                       & \cellcolor[HTML]{93C47D}20.07                                                                    \\
NSDF MLP                       & (1823;2;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}41.37                                                               & \cellcolor[HTML]{E06666}72.98                                                              & 260                                                                       & \cellcolor[HTML]{93C47D}10.34                                                                      & \cellcolor[HTML]{93C47D}18.14                                                                    \\
NVR low res. densegrid        & (403;2;1)/(512;1;1)                    & \cellcolor[HTML]{93C47D}22.71                                                               & \cellcolor[HTML]{E06666}69.16                                                              & 48                                                                        & \cellcolor[HTML]{93C47D}6.29                                                                       & \cellcolor[HTML]{93C47D}22.71                                                                    \\
NVR MLP                       & (403;2;1)/(512;1;1)                    & \cellcolor[HTML]{6AA84F}39.2                                                                & \cellcolor[HTML]{E06666}66.58                                                              & 48                                                                        & \cellcolor[HTML]{93C47D}12.11                                                                      & \cellcolor[HTML]{93C47D}20.48                                                                    \\
GIA low res. densegrid        & (4050;2;1)/(512;1;1)                   & \cellcolor[HTML]{E06666}66.15                                                               & \cellcolor[HTML]{E06666}59.12                                                              & 1                                                                         & \cellcolor[HTML]{E06666}66.15                                                                      & \cellcolor[HTML]{E06666}59.12                                                                    \\
GIA MLP                       & (4050;2;1)/(512;1;1)                   & \cellcolor[HTML]{6AA84F}42.87                                                               & \cellcolor[HTML]{E06666}73.02                                                              & 1                                                                         & \cellcolor[HTML]{6AA84F}42.87                                                                      & \cellcolor[HTML]{E06666}73.02                                                                    \\ \bottomrule
\end{tabular}
\end{table}






